Supervising Sound Localization by In-the-wild Egomotion

We present a method for learning binaural sound localization using egomotion as a supervisory signal. Over the course of a video, the cameras direction to a sound source will change as the camera moves. We train an audio model to predict sound directions that are consistent with visual estimates of camera motion, which we obtain using traditional methods from multi-view geometry. This provides a weak but plentiful form of supervision that we combine with traditional binaural cues. To evaluate this method, we propose a dataset of real-world audio-visual videos with egomotion. We show that our model can successfully learn from real-world data and that it performs well on sound localization tasks

==> tables/application.tex <==
\begin{table}[ht]
\centering
\caption{Multiple sound sources localization in synthetic dataset}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc}
    \toprule
    \multirow{2}{*}{Model}      
     & \multicolumn{3}{c}{One Source} & \multicolumn{3}{c}{One Dominant + Side} & \multicolumn{3}{c}{Two Dominant Source} & \multicolumn{3}{c}{Three Dominant Source}\\
      \cmidrule(lr){2-4}  \cmidrule(lr){5-7}  \cmidrule(lr){8-10}  \cmidrule(lr){11-13}& MAE(\degree)$\downarrow$ & 2clf & 8clf & MAE(\degree)$\downarrow$ &2clf &8clf  & MAE(\degree)$\downarrow$ &2clf &8clf & MAE(\degree)$\downarrow$ &2clf &8clf\\
    \midrule
    chance & 39.4 &49.0\% &15.0\% &39.4 &49.0\% &15.0\% &39.4 &49.0\% &15.0\% & 39.4 &49.0\% &15.0\% \\
    IID &  - &97.4\% &- &  - &87.0\% &- &  - &74.5\% &- & ? & ? & ?\\
    GTRot~\cite{chen2023sound} &4.3 &97.5\% &84.7\% & 22.5 &83.5\% &33.5\% & 30.2 &72.2\%&23.0\% & ? & ? & ?\\
    Ours-IIDonly & 22.2 &99.0\% &35.7\% & 47.2 &50.7\% &13.7\% & ? & ? & ? & ? & ? & ?\\
    \cdashlinelr{1-13} 
    % Ours-Tonly & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ?\\
    % Ours-Ronly & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? \\
    Ours-R\&T\&B & 9.8 &98.3\% &63.4\% & \textbf{23.2} &\textbf{87.2\%} &\textbf{36.2\%} & ? & ? & ?\\
    \midrule
    Supervised  & 2.8 &98.7\% &89.8\% & 10.8 & 91.8\% & 70.2\% & ? & ? & ? & ? & ? & ?\\
    \bottomrule
\end{tabular}
}
\end{table}
